3D-GRAND: A Million-Scale Dataset for 3D-LLMs with Better Grounding and Less Hallucination

The integration of language and 3D perception is crucial for embodied agents and robots that comprehend and interact with the physical world. While large language models (LLMs) have demonstrated impressive language understanding and generation capabilities, their adaptation to 3D environments (3D-LLMs) remains in its early stages. A primary challenge is a lack of large-scale datasets with dense grounding between language and 3D scenes. We introduce 3D-GRAND, a pioneering large-scale dataset comprising 40,087 household scenes paired with 6.2 million densely-grounded scene-language instructions. Our results show that instruction tuning with 3D-GRAND significantly enhances grounding capabilities and reduces hallucinations in 3D-LLMs. As part of our contributions, we propose a comprehensive benchmark 3D-POPE to systematically evaluate hallucination in 3D-LLMs, enabling fair comparisons of models. Our experiments highlight a scaling effect between dataset size and 3D-LLM performance, emphasizing the importance of large-scale 3D-text datasets for embodied AI research. Our results demonstrate early signals for effective sim-to-real transfer, indicating that models trained on large synthetic data can perform well on real-world 3D scans. Through 3D-GRAND and 3D-POPE, we aim to equip the embodied AI community with resources and insights to lead to more reliable and better-grounded 3D-LLMs. Project website: https://3d-grand.github.io

==> floating/tab_license.tex <==
\begin{table}[!h]
\centering 
\begin{tabular}{lll}
    \toprule
    Data Sources  & URL & License   \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-3}
    3D-Front  &  \href{https://tianchi.aliyun.com/dataset/65347}{Link} & CC BY 4.0 \\
    Structured3D  &   \href{https://structured3d-dataset.org/#license}{Link}  &  \href{https://drive.google.com/file/d/13ZwWpU_557ZQccwOUJ8H5lvXD7MeZFMa/view}{Structured3D Terms of Use} \\
    \midrule
    Software Code & URL & License   \\
    GPT-4/4V &  \href{https://chatgpt.com/}{Link} &  \href{https://openai.com/policies/terms-of-use/}{OpenAI Term of Use} \\
    \midrule
    Our Dataset Code & URL & License   \\
    3D-GRAND &  \href{https://3d-grand.github.io/}{Link} &  CC BY 4.0 \\
    3D-POPE &  \href{https://3d-grand.github.io/}{Link} &  CC BY 4.0 \\
    \bottomrule
\end{tabular}
\vspace*{-8pt}
\caption{License information for the scientific artifacts used and produced. \vspace*{-20pt}}
\label{tab:license}
\end{table}

==> sec/4_model.tex <==
\section{Model}

==> sec/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} Our claims are validated using experimental results on 3D-POPE and ScanRefer in Section~\ref{sec:experiments}.
  \item Did you describe the limitations of your work? \\
    \answerYes{} Limitations are discussed in the Supplementary Material.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} Potential negative societal impacts of our work are discussed in the Supplementary Material.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{The authors have reviewed NeurIPS Code of Ethics and do not notice any violations.} 
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{The paper does not include theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{The paper does not include theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code, data and instructions can be found on \url{https://3d-grand.github.io/}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We include implementation details in section~\ref{sec:implementation_details} and other model training details in the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our experiments are computationally heavy. For instance, fine-tuning the 3D LLM requires 576 GPU hours on an NVIDIA A40. We do not have sufficient computing resources to run it multiple times and report error bars. In addition, our performance increase on both grounding capability and hallucination reduction is quite big compared to existing methods, suggesting there is a high chance that our results and claims are statistically significant if we could afford multiple runs.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \\
    \answerYes{Implementation details can be found in the section~\ref{sec:implementation_details}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators? \\
    \answerYes{Existing assets are properly cited.}
  \item Did you mention the license of the assets? \\
    \answerYes{We include license of the assets in the supplementary material.} ]]
  \item Did you include any new assets either in the supplemental material or as a URL? \\
    \answerYes{In \url{https://3d-grand.github.io/}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating? \\
    \answerYes{We use publicly available datasets with open source license.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \\
    \answerYes{The data do not contain personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{We have included the full text of instructions given to participants and screenshots in the supplementary material.} \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We believe there are minimal to no risks to the annotators. The company was hired for annotation services, not for human subjects experiments; therefore, no IRB approval was required. At no point were we studying or directly intervening with the annotators.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Estimating an hourly wage is challenging due to the platform used. On average, we paid \$20 per thousand tasks. Our task is straightforward, requiring participants to select from binary answers with an additional option to choose “cannot decide.”}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
